A Generative Modeling Framework for Inferring Families of Biomechanical Constitutive Laws in Data-Sparse Regimes

Quantifying biomechanical properties of the human vasculature could deepen our understanding of cardiovascular diseases. Standard nonlinear regression in constitutive modeling requires considerable high-quality data and an explicit form of the constitutive model as prior knowledge. By contrast, we propose a novel approach that combines generative deep learning with Bayesian inference to efficiently infer families of constitutive relationships in data-sparse regimes. Inspired by the concept of functional priors, we develop a generative adversarial network (GAN) that incorporates a neural operator as the generator and a fully-connected neural network as the discriminator. The generator takes a vector of noise conditioned on measurement data as input and yields the predicted constitutive relationship, which is scrutinized by the discriminator in the following step. We demonstrate that this framework can accurately estimate means and standard deviations of the constitutive relationships of the murine aorta using data collected either from model-generated synthetic data or ex vivo experiments for mice with genetic deficiencies. In addition, the framework learns priors of constitutive models without explicitly knowing their functional form, providing a new model-agnostic approach to learning hidden constitutive behaviors from data.

==> copy.tex <==
The aorta consists of three main layers: adventitia, media, and intima. The adventitia, the outer layer of the aorta, mainly consists of collagen fibers, fibroblasts, and other ground substances that collaboratively provide support to and enhance the stability of the aorta, particularly at high pressure. In the medial layer, elastic lamellae delimit intralamellar space that is made of smooth muscle cells and extracellular matrix with collagen fibrils oriented in the circumferential direction. Intima is the innermost layer of the aorta and does not play an important role in load bearing~\cite{roccabianca2014computational}. The interaction and association between many constituents, glycoproteins, and other components in the aorta together control and regulate the mechanical properties of the vascular system~\cite{karnik2003critical}. Malfunction of the components may lead to structural changes, remodeling, and maladptation of the vascular system, which can be observed as changes in biomechanical properties or even vascular diseases such as Marfan syndrome~\cite{humphrey2013possible}, Elhers-Danlos syndrome~\cite{byers2017diagnosis}, or many other diseases. Hence, to deepen our understanding in vascular diseases necessitates the development of constitutive modeling for biomaterials. 
